GenPIP: In-Memory Acceleration of Genome Analysis via Tight Integration of Basecalling and Read Mapping

Nanopore sequencing is a widely-used high-throughput genome sequencing technology that can sequence long fragments of a genome into raw electrical signals at low cost. Nanopore sequencing requires two computationally-costly processing steps for accurate downstream genome analysis. The first step, basecalling, translates the raw electrical signals into nucleotide bases (i.e., A, C, G, T). The second step, read mapping, finds the correct location of a read in a reference genome. In existing genome analysis pipelines, basecalling and read mapping are executed separately. We observe in this work that such separate execution of the two most time-consuming steps inherently leads to (1) significant data movement and (2) redundant computations on the data, slowing down the genome analysis pipeline. This paper proposes GenPIP, an in-memory genome analysis accelerator that tightly integrates basecalling and read mapping. GenPIP improves the performance of the genome analysis pipeline with two key mechanisms: (1) in-memory fine-grained collaborative execution of the major genome analysis steps in parallel; (2) a new technique for early-rejection of low-quality and unmapped reads to timely stop the execution of genome analysis for such reads, reducing inefficient computation. Our experiments show that, for the execution of the genome analysis pipeline, GenPIP provides 41.6X (8.4X) speedup and 32.8X (20.8X) energy savings with negligible accuracy loss compared to the state-of-the-art software genome analysis tools executed on a state-of-the-art CPU (GPU). Compared to a design that combines state-of-the-art in-memory basecalling and read mapping accelerators, GenPIP provides 1.39X speedup and 1.37X energy savings.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> files/3.motivation.tex <==
%\section{Motivation and Challenge}~\label{sec:motivation}

We motivate building \name by making five main observations and analyzing the limitation of existing works.
Regardless of the sequencing technology, the current genome sequencing pipelines typically include two main steps: (1) genome sequencing and (2) data analysis. 
These two steps are separated from each other, which means the genomic reads generated by the genome sequencing machine in the "wet" lab have to be stored in the storage unit first and then read out for the computational analyses in the "dry" lab using clusters, supercomputers, or cloud computing~\cite{minion,illumina}.
The figure shows the sequencing and data analysis pipeline of MinION~\cite{minion} as an example of such sequencing pipelines. 
The MinION sequencing device requires a connection to a personal computer (PC) to start sequencing. The sequencing step should be followed by first a computational basecalling step and then subsequent computational analyses that can be done on the same PC, following the sequencing, or on the cloud (e.g., Amazon Web Services). 
However, such a pipeline has several limitations and drawbacks that make it \emph{unsuitable} for efficiently handling large-scale genomic studies. Next, we provide our analysis of these inefficiencies and conclude with the need for \name. 


\subsection{Revisiting Genome Sequencing and Read Mapping Pipeline}~\label{sec:gspipeline}
\textbf{Existing genome sequencing pipelines are \textit{inefficient} based on our five key observations}. 

\textbf{Observation 1}. Modern sequencing machines generate reads at an exponentially higher rate than prior sequencing technologies, with their growth far outpacing the growth in computational power in recent years. This is mainly due to dedicated specialized machines for sequencing and general-purpose machines (e.g., PCs) for computational analysis. The sequencing step is performed only once per genomic sample, but the subsequent analyses are performed repeatedly for different studies and different parameters~\cite{mangul2019systematic, wratten2021reproducible}. This motivates us to accelerate genome analysis using specialized hardware.

\textbf{Observation 2}. Basecalling and read mapping are two of the most time-consuming computational steps in the entire sequencing pipeline, and they are separated from each other in the current procedure.
The isolation between the sequencing and data analysis prevents real-time analysis, which is crucial for time-sensitive, life-saving applications~\cite{farnaes2018rapid, kingsmore2020measurement, clark2019diagnosis}. 
For example, the device control and data acquisition steps in the entire pipeline take $\sim432$ hours,  the basecalling step takes $\sim3100$ CPU hours, and the data analysis step takes $\sim580$ CPU hours, with $\sim500$ CPU hours for read mapping and $\sim80$ CPU hours for variant calling ~\cite{bowden2019sequencing}. 
This motivates us to accelerate two key computational steps, in specific basecalling and read alignment.


\textbf{Observation 3}.
A significant portion of the basecalled data is not needed for the subsequent analyses due to at least one of the following two reasons: 1) having low read quality and 2) being significantly different from the reference genome that is mapped to. 
It is highly recommended to use only genomic reads whose quality score is not less than seven~\cite{fukasawa2020longqc,leger2019pycoqc}. 
This flags at least 10-20\% of the read set as low-quality reads~\cite{bowden2019sequencing}, which will not be considered for further processing.
Figure~\ref{fig:ecoli} shows an example of quality score distribution of Escherichia coli (i.e., E. coli) genome dataset~\cite{ecoli}, where massive reads are basecalled but discarded, including very long reads.
Regardless of the exact value of such filtering threshold, such \dc{read quality control} step is performed only after completing the basecalling step.
Performing basecalling for the complete sequence of low-quality reads is computationally expensive as such reads will be discarded.
Therefore, by enabling analysis inside the sequencing machine, we have the opportunity to find the low-quality reads by basecalling small subsequences of the read and discard them quickly.

\begin{figure}[htbp]
%\vspace{-1em}
    \centering
    \includegraphics[scale=0.24]{figures/ecoli.pdf}
%\vspace{-1.5em}
    \caption{Read Quality Score Distribution of E. coli (Red Columns Represent The Number of Reads).}
    \label{fig:ecoli}
\end{figure}

Moreover, the similarity between each read and subsequence of the subject reference genome is examined after basecalling. 
If they are similar, then an alignment score (AS) tag is stored, indicating the similarity quality between the read and the chosen region of the reference genome~\cite{li2018minimap2}. 
If a read cannot be mapped to the reference genome, the AS tag is \texttt{NULL}. 
Unmapped reads cannot provide information for further genome analysis, but they have already been basecalled and executed mapping operations. 
For example, based on our analysis of the E. coli dataset~\cite{ecoli}, 30.5\% of all reads are unmapped (including low-quality reads). 
%This can be very high ($>$70\%) in metagenomic profiling studies~\cite{lapierre2020metalign}. 
Therefore, we have the opportunity to detect the unmapped reads early by tightly integrating read alignment computation nearby the basecalling.




\textbf{Observation 4}. The adoption of two separated steps generates a large amount of data movement between the sequencing machine and the compute machine performing the basecalling and/or the analysis, or even between different components of the same machine.
Most genome sequencing machines require network interface cards (NIC) to transfer data from the sequencing machine to other machines used for data analysis~\cite{minion,illumina}. 
Such data movement introduces two main issues.
1) Sequencing data is $10\times$ larger than the basecalled data for the same sample~\cite{minionrequirements}.
Transferring this data to the computing unit is time-consuming, costing from several tens of seconds to hundreds of seconds (using USB 3.0 as in MinION).
2) Moving a large amount of data through power-hungry buses consumes a significant amount of energy~\cite{lenkiewicz2018energy, boroumand2018google}.
Thus, moving data incurs high costs in terms of execution time and energy consumption~\cite{mutlu2020modern}. 
This motivates us to perform the computation inside the memory device to alleviate these costs and enable efficient analysis that can keep up with sequencing technologies.

\textbf{Observation 5} The use of cloud computing platforms (or remote machines for computing) is discouraged and sometimes disallowed in many countries due to data protection guidelines and potential security implications~\cite{naro2021side,faezi2019oligo, langmead2018cloud}.

Based on our five key observations, we conclude that it is essential to accelerate both basecalling and read mapping by reconsidering the pipeline and proposing an efficient hardware acceleration.


\subsection{NVM-based PIM for Genome Sequencing and Alignment}
NVM-based PIM is a promising solution to accelerate the basecalling~\cite{lou2020helix} and read alignment ~\cite{zokaee2018aligner,gupta2019rapid} as well as reduce the data movements and energy consumption by processing data in situ. 
However, previous works only focus on accelerating \emph{only} basecalling step~\cite{lou2020helix} or \emph{only} read alignment step~\cite{zokaee2018aligner,gupta2019rapid}, leaving these two steps separated from each other. In other words, the problems summarized in Section~\ref{sec:gspipeline} still exist.
Considering the sequencing machine has its own memory, we can enable the entire genome sequencing pipeline and alignment inside the sequencing machine using the NVM-based PIM techniques. 


However, 
enabling the entire pipeline inside the memory faces three main challenges as follows.  

\textbf{Meeting the demand of time-critical processing:}
Predicting low-quality and unmapped reads should be done as quickly as possible, avoiding unnecessary basecalling. Therefore, it is critical to (1) design high-performance PIM arrays for prediction and (2) reduce the communication overhead between the PIM arrays for prediction and the PIM arrays for basecalling.

\textbf{Satisfying the power and area budget:}
Both portable sequencing machines for real-time analysis~\cite{minion} and NVM-based PIM chips~\cite{lou2020helix} have power and area budget. Naively connecting existing accelerators for basecalling and read mapping cannot satisfy the budget. 

\textbf{Supporting variable read length:}
Previous NVM-based PIM works focus on the acceleration of short read alignment~\cite{zokaee2018aligner,gupta2019rapid,khatamifard2021genvom}. However, we need to flexibly support both short reads (for prediction) and long reads (regular processing) alignment in our work. %\srr{there is no long read support in existing works? even if it is fixed length?} \hycomment{They said they support but don't explain how.}


We conclude that an efficient in-memory genome analysis system is needed to mitigate the inefficiencies in current genome sequencing pipelines. Such a system should minimize unnecessary data movement and early reject low-quality and unmapped reads using minimal computation, supporting the unique properties (i.e., variable read length) of output data of the latest sequencing technologies.

==> ref-backup.tex <==
@comment{}}

@article{10.1093/gigascience/giy037,
 author = {Teng, Haotian and Cao, Minh Duc and Hall, Michael B and Duarte, Tania and Wang, Sheng and Coin, Lachlan J M},
 journal = {GigaScience},
 title = {{Chiron: Translating Nanopore Raw Signal Directly Into Nucleotide Sequence Using Deep Learning}},
 year = {2018}
}

@article{aguado-puig_accelerating_2022,
 author = {Aguado-Puig, Quim and Marco-Sola, Santiago and Moure, Juan Carlos and Castells-Rufas, David and Alvarez, Lluc and Espinosa, Antonio and Moreto, Miquel},
 journal = {IEEE Access},
 title = {{Accelerating Edit-distance Sequence Alignment On Gpu Using The Wavefront Algorithm}},
 year = {2022}
}

@article{aguado-puig_wfa-gpu_2022,
 author = {Aguado-Puig, Quim and Marco-Sola, Santiago and Moure, Juan Carlos and Matzoros, Christos and Castells-Rufas, David and Espinosa, Antonio and Moreto, Miquel},
 journal = {bioRxiv},
 title = {{Wfa-gpu: Gap-affine Pairwise Alignment Using Gpus}},
 year = {2022}
}

@article{alkan2009personalized,
 author = {Alkan, Can and Kidd, Jeffrey M and Marques-Bonet, Tomas and Aksay, Gozde and Antonacci, Francesca and Hormozdiari, Fereydoun and Kitzman, Jacob O and Baker, Carl and Malig, Maika and Mutlu, Onur and Sahinalp, S Cenk and Gibbs, Richard A and Eichler, Evan E},
 journal = {Nature Genetics},
 title = {{Personalized Copy Number And Segmental Duplication Maps Using Next-generation Sequencing}},
 year = {2009}
}

@article{alser2017gatekeeper,
 author = {Alser, Mohammed and Hassan, Hasan and Xin, Hongyi and Ergin, O{\u{g}}uz and Mutlu, Onur and Alkan, Can},
 journal = {Bioinformatics},
 title = {{Gatekeeper: A New Hardware Architecture For Accelerating Pre-alignment In Dna Short Read Mapping}},
 year = {2017}
}

@article{alser2017magnet,
 author = {Alser, Mohammed and Mutlu, Onur and Alkan, Can},
 journal = {arXiv},
 title = {{Magnet: Understanding And Improving The Accuracy Of Genome Pre-alignment Filtering}},
 year = {2017}
}

@article{alser2019shouji,
 author = {Alser, Mohammed and Hassan, Hasan and Kumar, Akash and Mutlu, Onur and Alkan, Can},
 journal = {Bioinformatics},
 title = {{Shouji: A Fast And Efficient Pre-alignment Filter For Sequence Alignment}},
 year = {2019}
}

@article{alser2020accelerating,
 author = {Alser, Mohammed and Bingöl, Zulal and Senol Cali, Damla and Kim, Jeremie and Ghose, Saugata and Alkan, Can and Mutlu, Onur},
 journal = {IEEE Micro},
 title = {{Accelerating Genome Analysis: A Primer On An Ongoing Journey}},
 year = {2020}
}

@article{alser2020sneakysnake,
 author = {Alser, Mohammed and Shahroodi, Taha and G{\'o}mez-Luna, Juan and Alkan, Can and Mutlu, Onur},
 journal = {Bioinformatics},
 title = {{Sneakysnake: A Fast And Accurate Universal Genome Pre-alignment Filter For Cpus, Gpus And Fpgas}},
 year = {2020}
}

@article{alser2020technology,
 author = {Alser, Mohammed and Rotman, Jeremy and Deshpande, Dhrithi and Taraszka, Kodi and Shi, Huwenbo and Baykal, Pelin Icer and Yang, Harry Taegyun and Xue, Victor and Knyazev, Sergey and Singer, Benjamin D. and Balliu, Brunilda and Koslicki, David and Skums, Pavel and Zelikovsky, Alex and Alkan, Can and Mutlu, Onur and Mangul, Serghei},
 journal = {Genome Biology},
 title = {{Technology Dictates Algorithms: Recent Developments In Read Alignment}},
 year = {2021}
}

@article{alser2021technology,
 author = {Alser, Mohammed and Rotman, Jeremy and Deshpande, Dhrithi and Taraszka, Kodi and Shi, Huwenbo and Baykal, Pelin Icer and Yang, Harry Taegyun and Xue, Victor and Knyazev, Sergey and Singer, Benjamin D and others},
 journal = {Genome biology},
 title = {{Technology Dictates Algorithms: Recent Developments In Read Alignment}},
 year = {2021}
}

@article{alser_molecules_2022,
 author = {Alser, Mohammed and Lindegger, Joel and Firtina, Can and Almadhoun, Nour and Mao, Haiyu and Singh, Gagandeep and Gomez-Luna, Juan and Mutlu, Onur},
 journal = {Computational and Structural Biotechnology Journal},
 title = {{From Molecules To Genomic Variations: Accelerating Genome Analysis Via Intelligent Algorithms And Architectures}},
 year = {2022}
}

@article{alvarez2017next,
 author = {Alvarez-Cubero, Maria Jesus and Saiz, Maria and Mart{\'\i}nez-Garc{\'\i}a, Bel{\'e}n and Sayalero, Sara M and Entrala, Carmen and Lorente, Jose Antonio and Martinez-Gonzalez, Luis Javier},
 journal = {Annals of Human Biology},
 title = {{Next Generation Sequencing: An Application In Forensic Sciences?}},
 year = {2017}
}

@article{amarasinghe2020opportunities,
 author = {Amarasinghe, Shanika L and Su, Shian and Dong, Xueyi and Zappia, Luke and Ritchie, Matthew E and Gouil, Quentin},
 journal = {Genome biology},
 title = {{Opportunities And Challenges In Long-read Sequencing Data Analysis}},
 year = {2020}
}

@inproceedings{angizi2020exploring,
 author = {Angizi, Shaahin and Zhang, Wei and Fan, Deliang},
 booktitle = {Proceedings of the 2020 on Great Lakes Symposium on VLSI},
 title = {{Exploring Dna Alignment-in-memory Leveraging Emerging Sot-mram}},
 year = {2020}
}

@inproceedings{angizi2020pim,
 author = {Angizi, Shaahin and Sun, Jiao and Zhang, Wei and Fan, Deliang},
 booktitle = {2020 {Design}, {Automation} {Test} in {Europe} {Conference} {Exhibition} ({DATE})},
 title = {{Pim-aligner: A Processing-in-mram Platform For Biological Sequence Alignment}},
 year = {2020}
}

@inproceedings{ankit2019puma,
 author = {Ankit, Aayush and Hajj, Izzat El and Chalamalasetti, Sai Rahul and Ndu, Geoffrey and Foltin, Martin and Williams, R Stanley and Faraboschi, Paolo and Hwu, Wen-mei W and Strachan, John Paul and Roy, Kaushik and others},
 booktitle = {Proceedings of the Twenty-Fourth International Conference on Architectural Support for Programming Languages and Operating Systems},
 title = {{Puma: A Programmable Ultra-efficient Memristor-based Accelerator For Machine Learning Inference}},
 year = {2019}
}

@article{ankit2020panther,
 author = {Ankit, Aayush and El Hajj, Izzat and Chalamalasetti, Sai Rahul and Agarwal, Sapan and Marinella, Matthew and Foltin, Martin and Strachan, John Paul and Milojicic, Dejan and Hwu, Wen-Mei and Roy, Kaushik},
 journal = {IEEE Transactions on Computers},
 title = {{Panther: A Programmable Architecture For Neural Network Training Harnessing Energy-efficient Reram}},
 year = {2020}
}

@inproceedings{arakawa2019multi,
 author = {Arakawa, Ren and Onizawa, Naoya and Diguet, Jean-Philippe and Hanyu, Takahiro},
 booktitle = {2019 26th IEEE International Conference on Electronics, Circuits and Systems (ICECS)},
 title = {{Multi-context Tcam Based Selective Computing Architecture For A Low-power Nn}},
 year = {2019}
}

@article{ardui2018single,
 author = {Ardui, Simon and Ameur, Adam and Vermeesch, Joris R and Hestand, Matthew S},
 journal = {Nucleic Acids Research},
 title = {{Single Molecule Real-time Smrt Sequencing Comes Of Age: Applications And Utilities For Medical Diagnostics}},
 year = {2018}
}

@article{Ashley2016,
 author = {Ashley, Euan A},
 journal = {Nature Reviews Genetics},
 title = {{Towards Precision Medicine}},
 year = {2016}
}

@inproceedings{behnam2018r,
 author = {Behnam, Payman and Chowdhury, Arjun Pal and Bojnordi, Mahdi Nazm},
 booktitle = {2018 IEEE 36th International Conference on Computer Design (ICCD)},
 title = {{R-cache: A Highly Set-associative In-package Cache Using Memristive Arrays}},
 year = {2018}
}

@article{belser2018chromosome,
 author = {Belser, Caroline and Istace, Benjamin and Denis, Erwan and Dubarry, Marion and Baurens, Franc-Christophe and Falentin, Cyril and Genete, Mathieu and Berrabah, Wahiba and Ch{\`e}vre, Anne-Marie and Delourme, R{\'e}gine and others},
 journal = {Nature plants},
 title = {{Chromosome-scale Assemblies Of Plant Genomes Using Nanopore Long Reads And Optical Maps}},
 year = {2018}
}

@article{bloom2021massively,
 author = {Bloom, Joshua S and Sathe, Laila and Munugala, Chetan and Jones, Eric M and Gasperini, Molly and Lubock, Nathan B and Yarza, Fauna and Thompson, Erin M and Kovary, Kyle M and Park, Jimin and others},
 journal = {Nature Biomedical Engineering},
 title = {{Massively Scaled-up Testing For Sars-cov-2 Rna Via Next-generation Sequencing Of Pooled And Barcoded Nasal And Saliva Samples}},
 year = {2021}
}

@misc{bonito,
 note = {\url{https://github.com/nanoporetech/bonito}},
 title = {{A Pytorch Basecaller For Oxford Nanopore Reads}}
}

@inproceedings{boroumand2018google,
 author = {Boroumand, Amirali and Ghose, Saugata and Kim, Youngsok and Ausavarungnirun, Rachata and Shiu, Eric and Thakur, Rahul and Kim, Daehyun and Kuusela, Aki and Knies, Allan and Ranganathan, Parthasarathy and others},
 booktitle = {Proceedings of the Twenty-Third International Conference on Architectural Support for Programming Languages and Operating Systems},
 title = {{Google Workloads For Consumer Devices: Mitigating Data Movement Bottlenecks}},
 year = {2018}
}

@article{borsting2015next,
 author = {B{\o}rsting, Claus and Morling, Niels},
 journal = {Forensic Science International: Genetics},
 title = {{Next Generation Sequencing And Its Applications In Forensic Genetics}},
 year = {2015}
}

@article{bowden2019sequencing,
 author = {Bowden, Rory and Davies, Robert W and Heger, Andreas and Pagnamenta, Alistair T and de Cesare, Mariateresa and Oikkonen, Laura E and Parkes, Duncan and Freeman, Colin and Dhalla, Fatima and Patel, Smita Y and others},
 journal = {Nature communications},
 title = {{Sequencing Of Human Genomes With Nanopore Technology}},
 year = {2019}
}

@article{boza_deepnano_2017,
 author = {Boža, Vladimír and Brejová, Broňa and Vinař, Tomáš},
 journal = {PLOS ONE},
 title = {{Deepnano: Deep Recurrent Neural Networks For Base Calling In Minion Nanopore Reads}},
 year = {2017}
}

@article{cali2017nanopore,
 author = {Senol Cali, Damla and Kim, Jeremie S and Ghose, Saugata and Alkan, Can and Mutlu, Onur},
 journal = {Briefings in Bioinformatics},
 title = {{Nanopore Sequencing Technology And Tools For Genome Assembly: Computational Analysis Of The Current State, Bottlenecks And Future Directions}},
 year = {2018}
}

@inproceedings{cali2020genasm,
 author = {Senol Cali, Damla and Kalsi, Gupreet and Bing{\"o}l, Zulal and Subramanian, Lavanya and Firtina, Can and Kim, Jeremie and Ausavarungnirun, Rachata and Alser, Mohammed and Nori, Anant and Luna, Juan and others},
 booktitle = {MICRO},
 title = {{Genasm: A High-performance, Low-power Approximate String Matching Acceleration Framework For Genome Sequence Analysis}},
 year = {2020}
}

@inproceedings{cali_segram_2022,
 author = {Senol Cali, Damla and Kanellopoulos, Konstantinos and Lindegger, Joël and Bingöl, Zülal and Kalsi, Gurpreet S. and Zuo, Ziyi and Firtina, Can and Cavlak, Meryem Banu and Kim, Jeremie and Ghiasi, Nika Mansouri and Singh, Gagandeep and Gómez-Luna, Juan and Alserr, Nour Almadhoun and Alser, Mohammed and Subramoney, Sreenivas and Alkan, Can and Ghose, Saugata and Mutlu, Onur},
 booktitle = {Proceedings of the 49th {Annual} {International} {Symposium} on {Computer} {Architecture}},
 title = {{Segram: A Universal Hardware Accelerator For Genomic Sequence-to-graph And Sequence-to-sequence Mapping}},
 year = {2022}
}

@article{chang20173t1r,
 author = {Chang, Meng-Fan and Lin, Chien-Chen and Lee, Albert and Chiang, Yen-Ning and Kuo, Chia-Chen and Yang, Geng-Hau and Tsai, Hsiang-Jen and Chen, Tien-Fu and Sheu, Shyh-Shyuan},
 journal = {IEEE Journal of Solid-State Circuits},
 title = {{A 3t1r Nonvolatile Tcam Using Mlc Reram For Frequent-off Instant-on Filters In Iot And Big-data Processing}},
 year = {2017}
}

@article{chen2013hybrid,
 author = {Chen, Yupeng and Schmidt, Bertil and Maskell, Douglas L},
 journal = {BMC bioinformatics},
 title = {{A Hybrid Short Read Mapping Accelerator}},
 year = {2013}
}

@inproceedings{chen2020parc,
 author = {Chen, Fan and Song, Linghao and Chen, Yiran and others},
 booktitle = {2020 25th Asia and South Pacific Design Automation Conference (ASP-DAC)},
 title = {{Parc: A Processing-in-cam Architecture For Genomic Long Read Pairwise Alignment Using Reram}},
 year = {2020}
}

@article{chi2016prime,
 author = {Chi, Ping and Li, Shuangchen and Xu, Cong and Zhang, Tao and Zhao, Jishen and Liu, Yongpan and Wang, Yu and Xie, Yuan},
 journal = {ACM SIGARCH Computer Architecture News},
 title = {{Prime: A Novel Processing-in-memory Architecture For Neural Network Computation In Reram-based Main Memory}},
 year = {2016}
}

@article{chin2011cancer,
 author = {Chin, Lynda and Andersen, Jannik N and Futreal, P Andrew},
 journal = {Nature Medicine},
 title = {{Cancer Genomics: From Discovery Science To Personalized Medicine}},
 year = {2011}
}

@article{clark2019diagnosis,
 author = {Clark, Michelle M and Hildreth, Amber and Batalov, Sergey and Ding, Yan and Chowdhury, Shimul and Watkins, Kelly and Ellsworth, Katarzyna and Camp, Brandon and Kint, Cyrielle I and Yacoubian, Calum and others},
 journal = {Science translational medicine},
 title = {{Diagnosis Of Genetic Diseases In Seriously Ill Children By Rapid Whole-genome Sequencing And Automated Phenotyping And Interpretation}},
 year = {2019}
}

@article{clarke2009continuous,
 author = {Clarke, James and Wu, Hai-Chen and Jayasinghe, Lakmal and Patel, Alpesh and Reid, Stuart and Bayley, Hagan},
 journal = {Nature nanotechnology},
 title = {{Continuous Base Identification For Single-molecule Nanopore Dna Sequencing}},
 year = {2009}
}

@misc{cpu,
 note = {\url{https://www.intel.com/content/dam/www/public/us/en/documents/white-papers/ia-introduction-basics-paper.pdf}},
 title = {{Introduction To Intel Architecture}},
 year = {2016}
}

@article{de2018nanopack,
 author = {De Coster, Wouter and D’hert, Svenn and Schultz, Darrin T and Cruts, Marc and Van Broeckhoven, Christine},
 journal = {Bioinformatics},
 title = {{Nanopack: Visualizing And Processing Long-read Sequencing Data}},
 year = {2018}
}

@article{de2021towards,
 author = {De Coster, Wouter and Weissensteiner, Matthias H and Sedlazeck, Fritz J},
 journal = {Nature Reviews Genetics},
 title = {{Towards Population-scale Long-read Sequencing}},
 year = {2021}
}

@inproceedings{deng2016multi,
 author = {Deng, Erya and Anghel, Lorena and Prenat, Guillaume and Zhao, Weisheng},
 booktitle = {2016 IEEE/ACM International Symposium on Nanoscale Architectures (NANOARCH)},
 title = {{Multi-context Non-volatile Content Addressable Memory Using Magnetic Tunnel Junctions}},
 year = {2016}
}

@article{diab2022framework,
 author = {Diab, Safaa and Nassereldine, Amir and Alser, Mohammed and G{\'o}mez-Luna, Juan and Mutlu, Onur and Hajj, Izzat El},
 journal = {arXiv preprint arXiv:2208.01243},
 title = {{A Framework For High-throughput Sequence Alignment Using Real Processing-in-memory Systems}},
 year = {2022}
}

@article{dong2012nvsim,
 author = {Dong, Xiangyu and Xu, Cong and Xie, Yuan and Jouppi, Norman P},
 journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
 title = {{Nvsim: A Circuit-level Performance, Energy, And Area Model For Emerging Nonvolatile Memory}},
 year = {2012}
}

@inproceedings{dunn2021squigglefilter,
 author = {Dunn, Tim and Sadasivan, Harisankar and Wadden, Jack and Goliya, Kush and Chen, Kuan-Yu and Blaauw, David and Das, Reetuparna and Narayanasamy, Satish},
 booktitle = {MICRO-54: 54th Annual IEEE/ACM International Symposium on Microarchitecture},
 title = {{Squigglefilter: An Accelerator For Portable Virus Detection}},
 year = {2021}
}

@misc{ecoli,
 author = {Nicholas J. Loman},
 note = {\url{http://lab.loman.net/2016/07/30/nanopore-r9-data-release/}},
 title = {{Nanopore R9 Rapid Run Data Release}},
 year = {2016}
}

@misc{ecoli_dataset,
 note = {\url{http://lab.loman.net/2016/07/30/nanopore-r9-data-release/}},
 title = {{Nanopore R9 Rapid Run Data Release}}
}

@article{eddy2004dynamic,
 author = {Eddy, Sean R},
 journal = {Nature biotechnology},
 title = {{What Is Dynamic Programming?}},
 year = {2004}
}

@article{ellegren2014genome,
 author = {Ellegren, Hans},
 journal = {Trends in Ecology \& Evolution},
 title = {{Genome Sequencing And Population Genomics In Non-model Organisms}},
 year = {2014}
}

@article{ellegren2016determinants,
 author = {Ellegren, Hans and Galtier, Nicolas},
 journal = {Nature Reviews Genetics},
 title = {{Determinants Of Genetic Diversity}},
 year = {2016}
}

@misc{ena,
 note = {\url{https://www.ebi.ac.uk/ena/browser/home}},
 title = {{European Nucleotide Archive}}
}

@article{ewing_base-calling_1998,
 author = {Ewing, Brent and Green, Phil},
 journal = {Genome Research},
 title = {{Base-calling Of Automated Sequencer Traces Using Phred. Ii. Error Probabilities}},
 year = {1998}
}

@inproceedings{faezi2019oligo,
 author = {Faezi, Sina and Chhetri, Sujit Rokka and Malawade, Arnav Vaibhav and Chaput, John Charles and Grover, William and Brisk, Philip and Al Faruque, Mohammad Abdullah},
 booktitle = {Network and Distributed Systems Security (NDSS) Symposium 2019},
 title = {{Oligo-snoop: A Non-invasive Side Channel Attack Against Dna Synthesis Machines}},
 year = {2019}
}

@article{farnaes2018rapid,
 author = {Farnaes, Lauge and Hildreth, Amber and Sweeney, Nathaly M and Clark, Michelle M and Chowdhury, Shimul and Nahas, Shareef and Cakici, Julie A and Benson, Wendy and Kaplan, Robert H and Kronick, Richard and others},
 journal = {NPJ genomic medicine},
 title = {{Rapid Whole-genome Sequencing Decreases Infant Morbidity And Cost Of Hospitalization}},
 year = {2018}
}

@inproceedings{feng2019accelerating,
 author = {Feng, Zonghao and Qiu, Shuang and Wang, Lipeng and Luo, Qiong},
 booktitle = {Proceedings of the 48th International Conference on Parallel Processing},
 title = {{Accelerating Long Read Alignment On Three Processors}},
 year = {2019}
}

@article{firtina2020apollo,
 author = {Firtina, Can and Kim, Jeremie S and Alser, Mohammed and Senol Cali, Damla and Cicek, A Ercument and Alkan, Can and Mutlu, Onur},
 journal = {Bioinformatics},
 title = {{Apollo: A Sequencing-technology-independent, Scalable And Accurate Assembly Polishing Algorithm}},
 year = {2020}
}

@article{firtina_aphmm_2022,
 author = {Firtina, Can and Pillai, Kamlesh and Kalsi, Gurpreet S. and Suresh, Bharathwaj and Cali, Damla Senol and Kim, Jeremie and Shahroodi, Taha and Cavlak, Meryem Banu and Lindegger, Joel and Alser, Mohammed and Luna, Juan Gómez and Subramoney, Sreenivas and Mutlu, Onur},
 journal = {arXiv preprint arXiv:2207.09765},
 title = {{Aphmm: Accelerating Profile Hidden Markov Models For Fast And Energy-efficient Genome Analysis}},
 year = {2022}
}

@article{firtina_blend_2021,
 author = {Firtina, Can and Park, Jisung and Kim, Jeremie S. and Alser, Mohammed and Senol Cali, Damla and Shahroodi, Taha and Ghiasi, Nika Mansouri and Singh, Gagandeep and Kanellopoulos, Konstantinos and Alkan, Can and Mutlu, Onur},
 journal = {arXiv preprint arXiv:2112.08687},
 title = {{Blend: A Fast, Memory-efficient, And Accurate Mechanism To Find Fuzzy Seed Matches}},
 year = {2021}
}

@misc{Flappie,
 author = {Oxford Nanopore Technology},
 journal = {GitHub repository},
 note = {\url{https://github.com/nanoporetech/flappie}},
 title = {{Flappie}}
}

@article{flores2013p4,
 author = {Flores, Mauricio and Glusman, Gustavo and Brogaard, Kristin and Price, Nathan D and Hood, Leroy},
 journal = {Personalized Medicine},
 title = {{P4 Medicine: How Systems Medicine Will Transform The Healthcare Sector And Society}},
 year = {2013}
}

@inproceedings{fujiki2018genax,
 author = {Fujiki, Daichi and Subramaniyan, Arun and Zhang, Tianjun and Zeng, Yu and Das, Reetuparna and Blaauw, David and Narayanasamy, Satish},
 booktitle = {2018 ACM/IEEE 45th Annual International Symposium on Computer Architecture (ISCA)},
 title = {{Genax: A Genome Sequencing Accelerator}},
 year = {2018}
}

@article{fukasawa2020longqc,
 author = {Fukasawa, Yoshinori and Ermini, Luca and Wang, Hai and Carty, Karen and Cheung, Min-Sin},
 journal = {G3: Genes, Genomes, Genetics},
 title = {{Longqc: A Quality Control Tool For Third Generation Sequencing Long Read Data}},
 year = {2020}
}

@article{gamaarachchi2022fast,
 author = {Gamaarachchi, Hasindu and Samarakoon, Hiruna and Jenner, Sasha P and Ferguson, James M and Amos, Timothy G and Hammond, Jillian M and Saadat, Hassaan and Smith, Martin A and Parameswaran, Sri and Deveson, Ira W},
 journal = {Nature Biotechnology},
 title = {{Fast Nanopore Sequencing Data Analysis With Slow5}},
 year = {2022}
}

@article{ghose2019processing,
 author = {Ghose, Saugata and Boroumand, Amirali and Kim, Jeremie S and G{\'o}mez-Luna, Juan and Mutlu, Onur},
 journal = {IBM Journal of Research and Development},
 title = {{Processing-in-memory: A Workload-driven Perspective}},
 year = {2019}
}

@article{gilchrist2015whole,
 author = {Gilchrist, Carol A and Turner, Stephen D and Riley, Margaret F and Petri, William A and Hewlett, Erik L},
 journal = {Clinical Microbiology Reviews},
 title = {{Whole-genome Sequencing In Outbreak Analysis}},
 year = {2015}
}

@article{ginsburg2009genomic,
 author = {Ginsburg, Geoffrey S and Willard, Huntington F},
 journal = {Translational Research},
 title = {{Genomic And Personalized Medicine: Foundations And Applications}},
 year = {2009}
}

@article{giordano2017novo,
 author = {Giordano, Francesca and Aigrain, Louise and Quail, Michael A and Coupland, Paul and Bonfield, James K and Davies, Robert M and Tischler, German and Jackson, David K and Keane, Thomas M and Li, Jing and others},
 journal = {Scientific reports},
 title = {{De Novo Yeast Genome Assemblies From Minion, Pacbio And Miseq Platforms}},
 year = {2017}
}

@article{gire2014genomic,
 author = {Gire, Stephen K and Goba, Augustine and Andersen, Kristian G and Sealfon, Rachel SG and Park, Daniel J and Kanneh, Lansana and Jalloh, Simbirie and Momoh, Mambu and Fullah, Mohamed and Dudas, Gytis and others},
 journal = {science},
 title = {{Genomic Surveillance Elucidates Ebola Virus Origin And Transmission During The 2014 Outbreak}},
 year = {2014}
}

@article{gnawali2018low,
 author = {Gnawali, Krishna Prasad and Mozaffari, Seyed Nima and Tragoudas, Spyros},
 journal = {IEEE Transactions on Nanotechnology},
 title = {{Low Power Spintronic Ternary Content Addressable Memory}},
 year = {2018}
}

@misc{gpu,
 note = {\url{https://www.pny.com.tw/jp/upload/download_files/jp_download_list_19b22_wr2i3c5qid.pdf}},
 title = {{Nvidia Rtx Geforce 2080 Ti 11gb}},
 year = {2018}
}

@article{graves2020memory,
 author = {Graves, Catherine E and Li, Can and Sheng, Xia and Miller, Darrin and Ignowski, Jim and Kiyama, Lennie and Strachan, John Paul},
 journal = {Advanced Materials},
 title = {{In-memory Computing With Memristor Content Addressable Memories For Pattern Matching}},
 year = {2020}
}

@inproceedings{guo_hardware_2019,
 author = {Guo, Licheng and Lau, Jason and Ruan, Zhenyuan and Wei, Peng and Cong, Jason},
 booktitle = {2019 {IEEE} 27th {Annual} {International} {Symposium} on {Field}-{Programmable} {Custom} {Computing} {Machines} ({FCCM})},
 title = {{Hardware Acceleration Of Long Read Pairwise Overlapping In Genome Sequencing: A Race Between Fpga And Gpu}},
 year = {2019}
}

@misc{Guppy,
 author = { Oxford Nanopore Technology},
 journal = {GitHub repository},
 note = {\url{https://denbi-nanopore-training-course.readthedocs.io/en/latest/basecalling/basecalling.html }},
 title = {{Guppy}}
}

@article{gupta2019nnpim,
 author = {Gupta, Saransh and Imani, Mohsen and Kaur, Harveen and Rosing, Tajana Simunic},
 journal = {IEEE Transactions on Computers},
 title = {{Nnpim: A Processing In-memory Architecture For Neural Network Acceleration}},
 year = {2019}
}

@inproceedings{gupta2019rapid,
 author = {Gupta, Saransh and Imani, Mohsen and Khaleghi, Behnam and Kumar, Venkatesh and Rosing, Tajana},
 booktitle = {ISLPED},
 title = {{Rapid: A Reram Processing In-memory Architecture For Dna Sequence Alignment}},
 year = {2019}
}

@inproceedings{haghi_fpga_2021,
 author = {Haghi, Abbas and Marco-Sola, Santiago and Alvarez, Lluc and Diamantopoulos, Dionysios and Hagleitner, Christoph and Moreto, Miquel},
 booktitle = {2021 31st {International} {Conference} on {Field}-{Programmable} {Logic} and {Applications} ({FPL})},
 title = {{An Fpga Accelerator Of The Wavefront Algorithm For Genomics Pairwise Alignment}},
 year = {2021}
}

@article{halawani2019reram,
 author = {Halawani, Yasmin and Mohammad, Baker and Lebdeh, Muath Abu and Al-Qutayri, Mahmoud and Al-Sarawi, Said F},
 journal = {IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
 title = {{Reram-based In-memory Computing For Search Engine And Neural Network Applications}},
 year = {2019}
}

@article{hammad_scalable_2021,
 author = {Hammad, Karim and Wu, Zhongpan and Ghafar-Zadeh, Ebrahim and Magierowski, Sebastian},
 journal = {IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
 title = {{A Scalable Hardware Accelerator For Mobile Dna Sequencing}},
 year = {2021}
}

@article{hoban2016finding,
 author = {Hoban, Sean and Kelley, Joanna L and Lotterhos, Katie E and Antolin, Michael F and Bradburd, Gideon and Lowry, David B and Poss, Mary L and Reed, Laura K and Storfer, Andrew and Whitlock, Michael C},
 journal = {The American Naturalist},
 title = {{Finding The Genomic Basis Of Local Adaptation: Pitfalls, Practical Solutions, And Future Directions}},
 year = {2016}
}

@inproceedings{hoefler2017spin,
 author = {Hoefler, Torsten and Di Girolamo, Salvatore and Taranov, Konstantin and Grant, Ryan E and Brightwell, Ron},
 booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
 title = {{Spin: High-performance Streaming Processing In The Network}},
 year = {2017}
}

@inproceedings{huang2021mixed,
 author = {Huang, Sitao and Ankit, Aayush and Silveira, Plinio and Antunes, Rodrigo and Chalamalasetti, Sai Rahul and El Hajj, Izzat and Kim, Dong Eun and Aguiar, Glaucimar and Bruel, Pedro and Serebryakov, Sergey and others},
 booktitle = {2021 26th Asia and South Pacific Design Automation Conference (ASP-DAC)},
 title = {{Mixed Precision Quantization For Reram-based Dnn Inference Accelerators}},
 year = {2021}
}

@article{huang_sacall_2022,
 author = {Huang, Neng and Nie, Fan and Ni, Peng and Luo, Feng and Wang, Jianxin},
 journal = {IEEE/ACM Transactions on Computational Biology and Bioinformatics},
 title = {{Sacall: A Neural Network Basecaller For Oxford Nanopore Sequencing Data Based On Self-attention Mechanism}},
 year = {2022}
}

@misc{human_dataset,
 note = {\url{https://www.ebi.ac.uk/ena/browser/view/PRJEB30620}},
 title = {{European Nucleotide Archive -- Sequencing Of Human Genomes With Nanopore Technology}}
}

@misc{illumina,
 note = {\url{https://www.illumina.com/systems/sequencing-platforms/miniseq.html}},
 title = {{Illumina}}
}

@inproceedings{imani2016masc,
 author = {Imani, Mohsen and Patil, Shruti and Rosing, Tajana S},
 booktitle = {2016 Design, Automation \& Test in Europe Conference \& Exhibition (DATE)},
 title = {{Masc: Ultra-low Energy Multiple-access Single-charge Tcam For Approximate Computing}},
 year = {2016}
}

@article{imani2017multi,
 author = {Imani, Mohsen and Rahimi, Abbas and Mercati, Pietro and Rosing, Tajana Simunic},
 journal = {IEEE Transactions on Multi-Scale Computing Systems},
 title = {{Multi-stage Tunable Approximate Search In Resistive Associative Memory}},
 year = {2017}
}

@inproceedings{imani2019floatpim,
 author = {Imani, Mohsen and Gupta, Saransh and Kim, Yeseong and Rosing, Tajana},
 booktitle = {2019 ACM/IEEE 46th Annual International Symposium on Computer Architecture (ISCA)},
 title = {{Floatpim: In-memory Acceleration Of Deep Neural Network Training With High Precision}},
 year = {2019}
}

@article{jain2016oxford,
 author = {Jain, Miten and Olsen, Hugh E and Paten, Benedict and Akeson, Mark},
 journal = {Genome biology},
 title = {{The Oxford Nanopore Minion: Delivery Of Nanopore Sequencing To The Genomics Community}},
 year = {2016}
}

@article{jain2017minion,
 author = {Jain, Miten and Tyson, John R and Loose, Matthew and Ip, Camilla LC and Eccles, David A and O'Grady, Justin and Malla, Sunir and Leggett, Richard M and Wallerman, Ola and Jansen, Hans J and others},
 journal = {F1000Research},
 title = {{Minion Analysis And Reference Consortium: Phase 2 Data Release And Analysis Of R9. 0 Chemistry}},
 year = {2017}
}

@article{jain2018nanopore,
 author = {Jain, Miten and Koren, Sergey and Miga, Karen H and Quick, Josh and Rand, Arthur C and Sasani, Thomas A and Tyson, John R and Beggs, Andrew D and Dilthey, Alexander T and Fiddes, Ian T and others},
 journal = {Nature biotechnology},
 title = {{Nanopore Sequencing And Assembly Of A Human Genome With Ultra-long Reads}},
 year = {2018}
}

@inproceedings{jain2019accelerating,
 author = {Jain, Chirag and Misra, Sanchit and Zhang, Haowen and Dilthey, Alexander and Aluru, Srinivas},
 booktitle = {2019 IEEE International Parallel and Distributed Processing Symposium (IPDPS)},
 title = {{Accelerating Sequence Alignment To Graphs}},
 year = {2019}
}

@article{kaplan2017resistive,
 author = {Kaplan, Roman and Yavits, Leonid and Ginosar, Ran and Weiser, Uri},
 journal = {IEEE Micro},
 title = {{A Resistive Cam Processing-in-storage Architecture For Dna Sequence Alignment}},
 year = {2017}
}

@article{kaplan2018rassa,
 author = {Kaplan, Roman and Yavits, Leonid and Ginosar, Ran},
 journal = {IEEE Micro},
 title = {{Rassa: Resistive Prealignment Accelerator For Approximate Dna Long Read Mapping}},
 year = {2018}
}

@inproceedings{kaplan2020bioseal,
 author = {Kaplan, Roman and Yavits, Leonid and Ginosasr, Ran},
 booktitle = {Proceedings of the 13th ACM International Systems and Storage Conference},
 title = {{Bioseal: In-memory Biological Sequence Alignment Accelerator For Large-scale Genomic Data}},
 year = {2020}
}

@article{karam2015emerging,
 author = {Karam, Robert and Puri, Ruchir and Ghosh, Swaroop and Bhunia, Swarup},
 journal = {Proceedings of the IEEE},
 title = {{Emerging Trends In Design And Applications Of Memory-based Computing And Content-addressable Memories}},
 year = {2015}
}

@article{kchouk2017generations,
 author = {Kchouk, Mehdi and Gibrat, Jean-Francois and Elloumi, Mourad},
 journal = {Biology and Medicine},
 title = {{Generations Of Sequencing Technologies: From First To Next Generation}},
 year = {2017}
}

@article{khatamifard2017non,
 author = {Khatamifard, S Karen and Chowdhury, Zamshed and Pande, Nakul and Razaviyayn, Meisam and Kim, Chris and Karpuzcu, Ulya R},
 journal = {Scanning Electron Microsc Meet at},
 title = {{A Non-volatile Near-memory Read Mapping Accelerator}},
 year = {2017}
}

@article{khatamifard2021genvom,
 author = {Khatamifard, S Karen and Chowdhury, Zamshed and Pande, Nakul and Razaviyayn, Meisam and Kim, Chris H and Karpuzcu, Ulya R},
 journal = {IEEE/ACM Transactions on Computational Biology and Bioinformatics},
 title = {{Genvom: Read Mapping Near Non-volatile Memory}},
 year = {2021}
}

@article{kim2018grim,
 author = {Kim, Jeremie S. and Senol Cali, Damla and Xin, Hongyi and Lee, Donghyuk and Ghose, Saugata and Alser, Mohammed and Hassan, Hasan and Ergin, Oguz and Alkan, Can and Mutlu, Onur},
 journal = {BMC Genomics},
 title = {{Grim-filter: Fast Seed Location Filtering In Dna Read Mapping Using Processing-in-memory Technologies}},
 year = {2018}
}

@inproceedings{kim2018low,
 author = {Kim, Cheol and Sung, Rak-Joo and Ahn, Sung-Gi and Min, Jisu and Kwon, Kee-Won},
 booktitle = {2018 IEEE International Symposium on Circuits and Systems (ISCAS)},
 title = {{Low Power Search Engine Using Non-volatile Memory Based Tcam With Priority Encoding And Selective Activation Of Search Line And Match Line}},
 year = {2018}
}

@article{kim2019airlift,
 author = {Kim, Jeremie S and Firtina, Can and Cavlak, Meryem Banu and Cali, Damla Senol and Alser, Mohammed and Hajinazar, Nastaran and Alkan, Can and Mutlu, Onur},
 journal = {arXiv},
 title = {{Airlift: A Fast And Comprehensive Technique For Remapping Alignments Between Reference Genomes}},
 year = {2019}
}

@article{kim_fastremap_2022,
 author = {Kim, Jeremie S and Firtina, Can and Cavlak, Meryem Banu and Senol Cali, Damla and Alkan, Can and Mutlu, Onur},
 journal = {Bioinformatics},
 title = {{Fastremap: A Tool For Quickly Remapping Reads Between Genome Assemblies}},
 year = {2022}
}

@article{kingsmore2020measurement,
 author = {Kingsmore, Stephen F and Henderson, Audrey and Owen, Mallory J and Clark, Michelle M and Hansen, Christian and Dimmock, David and Chambers, Christina D and Jeliffe-Pawlowski, Laura L and Hobbs, Charlotte},
 journal = {NPJ genomic medicine},
 title = {{Measurement Of Genetic Diseases As A Cause Of Mortality In Infants Receiving Whole Genome Sequencing}},
 year = {2020}
}

@article{konishi_halcyon_2021,
 author = {Konishi, Hiroki and Yamaguchi, Rui and Yamaguchi, Kiyoshi and Furukawa, Yoichi and Imoto, Seiya},
 journal = {Bioinformatics},
 title = {{Halcyon: An Accurate Basecaller Exploiting An Encoder–decoder Model With Monotonic Attention}},
 year = {2021}
}

@article{kovaka2021targeted,
 author = {Kovaka, Sam and Fan, Yunfan and Ni, Bohan and Timp, Winston and Schatz, Michael C},
 journal = {Nature Biotechnology},
 title = {{Targeted Nanopore Sequencing By Real-time Mapping Of Raw Electrical Signal With Uncalled}},
 year = {2021}
}

@article{kwon2019three,
 author = {Kwon, Jimin and Takeda, Yasunori and Shiwaku, Rei and Tokito, Shizuo and Cho, Kilwon and Jung, Sungjune},
 journal = {Nature communications},
 title = {{Three-dimensional Monolithic Integration In Flexible Printed Organic Transistors}},
 year = {2019}
}

@inproceedings{laguna2020seed,
 author = {Laguna, Ann Franchesca and Gamaarachchi, Hasindu and Yin, Xunzhao and Niemier, Michael and Parameswaran, Sri and Hu, X Sharon},
 booktitle = {2020 IEEE/ACM International Conference On Computer Aided Design (ICCAD)},
 title = {{Seed-and-vote Based In-memory Accelerator For Dna Read Mapping}},
 year = {2020}
}

@article{langmead2018cloud,
 author = {Langmead, Ben and Nellore, Abhinav},
 journal = {Nature Reviews Genetics},
 title = {{Cloud Computing For Genomic Data Analysis And Collaboration}},
 year = {2018}
}

@article{lapierre2020metalign,
 author = {LaPierre, Nathan and Alser, Mohammed and Eskin, Eleazar and Koslicki, David and Mangul, Serghei},
 journal = {Genome biology},
 title = {{Metalign: Efficient Alignment-based Metagenomic Profiling Via Containment Min Hash}},
 year = {2020}
}

@article{le2013selected,
 author = {Le, Vien Thi Minh and Diep, Binh An},
 journal = {Current Opinion in Critical Care},
 title = {{Selected Insights From Application Of Whole Genome Sequencing For Outbreak Investigations}},
 year = {2013}
}

@article{leger2019pycoqc,
 author = {Leger, Adrien and Leonardi, Tommaso},
 journal = {Journal of Open Source Software},
 title = {{Pycoqc, Interactive Quality Control For Oxford Nanopore Sequencing}},
 year = {2019}
}

@article{lenkiewicz2018energy,
 author = {Lenkiewicz, Przemyslaw and Broekema, P Chris and Metzler, Bernard},
 journal = {Future Generation Computer Systems},
 title = {{Energy-efficient Data Transfers In Radio Astronomy With Software Udp Rdma}},
 year = {2018}
}

@inproceedings{lergan,
 author = {Mao, Haiyu and Song, Mingcong and Li, Tao and Dai, Yuting and Shu, Jiwu},
 booktitle = {Proceedings of the 51st Annual IEEE/ACM International Symposium on Microarchitecture},
 title = {{Lergan: A Zero-free, Low Data Movement And Pim-based Gan Architecture}},
 year = {2018}
}

@inproceedings{li20131mb,
 author = {Li, Jing and Montoye, Robert and Ishii, Masatoshi and Stawiasz, Kevin and Nishida, Takeshi and Maloney, Kim and Ditlow, Gary and Lewis, Scott and Maffitt, Tom and Jordan, Richard and others},
 booktitle = {2013 Symposium on VLSI Technology},
 title = {{1mb 0.41 $\mu$m 2 2t-2r Cell Nonvolatile Tcam With Two-bit Encoding And Clocked Self-referenced Sensing}},
 year = {2013}
}

@inproceedings{li2016nvsim,
 author = {Li, Shuangchen and Liu, Liu and Gu, Peng and Xu, Cong and Xie, Yuan},
 booktitle = {2016 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)},
 title = {{Nvsim-cam: A Circuit-level Simulator For Emerging Nonvolatile Memory Based Content-addressable Memory}},
 year = {2016}
}

@article{li2018minimap2,
 author = {Li, Heng},
 journal = {Bioinformatics},
 title = {{Minimap2: Pairwise Alignment For Nucleotide Sequences}},
 year = {2018}
}

@article{li2020analog,
 author = {Li, Can and Graves, Catherine E and Sheng, Xia and Miller, Darrin and Foltin, Martin and Pedretti, Giacomo and Strachan, John Paul},
 journal = {Nature communications},
 title = {{Analog Content-addressable Memories With Memristors}},
 year = {2020}
}

@article{lindner2017hilive,
 author = {Lindner, Martin S and Strauch, Benjamin and Schulze, Jakob M and Tausch, Simon H and Dabrowski, Piotr W and Nitsche, Andreas and Renard, Bernhard Y},
 journal = {Bioinformatics},
 title = {{Hilive: Real-time Mapping Of Illumina Reads While Sequencing}},
 year = {2017}
}

@article{logsdon2020long,
 author = {Logsdon, Glennis A and Vollger, Mitchell R and Eichler, Evan E},
 journal = {Nature Reviews Genetics},
 title = {{Long-read Human Genome Sequencing And Its Applications}},
 year = {2020}
}

@inproceedings{longlive,
 author = {Cai, Yi and Lin, Yujun and Xia, Lixue and Chen, Xiaoming and Han, Song and Wang, Yu and Yang, Huazhong},
 booktitle = {Proceedings of the 55th Annual Design Automation Conference},
 title = {{Long Live Time: Improving Lifetime For Training-in-memory Engines By Structured Gradient Sparsification}},
 year = {2018}
}

@article{lou2018brawl,
 author = {Lou, Qian and Jiang, Lei},
 journal = {IEEE Computer Architecture Letters},
 title = {{Brawl: A Spintronics-based Portable Basecalling-in-memory Architecture For Nanopore Genome Sequencing}},
 year = {2018}
}

@inproceedings{lou2020helix,
 author = {Lou, Qian and Janga, Sarath Chandra and Jiang, Lei},
 booktitle = {Proceedings of the ACM International Conference on Parallel Architectures and Compilation Techniques},
 title = {{Helix: Algorithm/architecture Co-design For Accelerating Nanopore Genome Base-calling}},
 year = {2020}
}

@inproceedings{lv_end--end_2020,
 author = {Lv, Xuan and Chen, Zhiguang and Lu, Yutong and Yang, Yuedong},
 booktitle = {2020 {IEEE} {International} {Conference} on {Bioinformatics} and {Biomedicine} ({BIBM})},
 title = {{An End-to-end Oxford Nanopore Basecaller Using Convolution-augmented Transformer}},
 year = {2020}
}

@article{mangul2019systematic,
 author = {Mangul, Serghei and Martin, Lana S and Hill, Brian L and Lam, Angela Ka-Mei and Distler, Margaret G and Zelikovsky, Alex and Eskin, Eleazar and Flint, Jonathan},
 journal = {Nature communications},
 title = {{Systematic Benchmarking Of Omics Computational Tools}},
 year = {2019}
}

@inproceedings{mansouri2022genstore,
 author = {Mansouri Ghiasi, Nika and Park, Jisung and Mustafa, Harun and Kim, Jeremie and Olgun, Ataberk and Gollwitzer, Arvid and Senol Cali, Damla and Firtina, Can and Mao, Haiyu and Almadhoun Alserr, Nour and Ausavarungnirun, Rachata and Vijaykumar, Nandita and Alser, Mohammed and Mutlu, Onur},
 booktitle = {Proceedings of the 27th {ACM} {International} {Conference} on {Architectural} {Support} for {Programming} {Languages} and {Operating} {Systems}},
 title = {{Genstore: A High-performance In-storage Processing System For Genome Sequence Analysis}},
 year = {2022}
}

@article{mao2020lrgan,
 author = {Mao, Haiyu and Shu, Jiwu and Song, Mingcong and Li, Tao},
 journal = {IEEE Transactions on Computers},
 title = {{Lrgan: A Compact And Energy Efficient Pim-based Architecture For Gan Training}},
 year = {2020}
}

@misc{minion,
 note = {\url{https://nanoporetech.com/products/minion}},
 title = {{Minion}}
}

@misc{minionrequirements,
 note = {\url{https://community.nanoporetech.com/requirements_documents/minion-it-reqs.pdf}},
 title = {{Minion Mk1b It Requirements}}
}

@inproceedings{mitchell2013using,
 author = {Mitchell, Christopher and Geng, Yifeng and Li, Jinyang},
 booktitle = {2013 $\{$USENIX$\}$ Annual Technical Conference ($\{$USENIX$\}$$\{$ATC$\}$ 13)},
 title = {{Using One-sided $\$rdma$\$ Reads To Build A Fast, Cpu-efficient Key-value Store}},
 year = {2013}
}

@article{mittal2019survey,
 author = {Mittal, Sparsh},
 journal = {Machine learning and knowledge extraction},
 title = {{A Survey Of Reram-based Architectures For Processing-in-memory And Neural Networks}},
 year = {2019}
}

@inproceedings{muralimanohar2007optimizing,
 author = {Muralimanohar, Naveen and Balasubramonian, Rajeev and Jouppi, Norm},
 booktitle = {40th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO 2007)},
 title = {{Optimizing Nuca Organizations And Wiring Alternatives For Large Caches With Cacti 6.0}},
 year = {2007}
}

@article{murigneux2020comparison,
 author = {Murigneux, Valentine and Rai, Subash Kumar and Furtado, Agnelo and Bruxner, Timothy JC and Tian, Wei and Harliwong, Ivon and Wei, Hanmin and Yang, Bicheng and Ye, Qianyu and Anderson, Ellis and others},
 journal = {GigaScience},
 title = {{Comparison Of Long-read Methods For Sequencing And Assembly Of A Plant Genome}},
 year = {2020}
}

@inproceedings{mutlu2019enabling,
 author = {Mutlu, Onur and Ghose, Saugata and G{\'o}mez-Luna, Juan and Ausavarungnirun, Rachata},
 booktitle = {Proceedings of the 56th Annual Design Automation Conference 2019},
 title = {{Enabling Practical Processing In And Near Memory For Data-intensive Computing}},
 year = {2019}
}

@article{mutlu2019processing,
 author = {Mutlu, Onur and Ghose, Saugata and G{\'o}mez-Luna, Juan and Ausavarungnirun, Rachata},
 journal = {Microprocessors and Microsystems},
 title = {{Processing Data Where It Makes Sense: Enabling In-memory Computation}},
 year = {2019}
}

@article{mutlu2020modern,
 author = {Mutlu, Onur and Ghose, Saugata and G{\'o}mez-Luna, Juan and Ausavarungnirun, Rachata},
 journal = {arXiv preprint arXiv:2012.03112},
 title = {{A Modern Primer On Processing In Memory}},
 year = {2020}
}

@inproceedings{nag2019gencache,
 author = {Nag, Anirban and Ramachandra, C. N. and Balasubramonian, Rajeev and Stutsman, Ryan and Giacomin, Edouard and Kambalasubramanyam, Hari and Gaillardon, Pierre-Emmanuel},
 booktitle = {Proceedings of the 52nd {Annual} {IEEE}/{ACM} {International} {Symposium} on {Microarchitecture}},
 title = {{Gencache: Leveraging In-cache Operators For Efficient Sequence Alignment}},
 year = {2019}
}

@article{naro2021side,
 author = {Naro, Daniel and Delgado, Jaime and Llorente, Silvia},
 journal = {Multimedia Tools and Applications},
 title = {{Side Channel Attack On A Partially Encrypted Mpeg-g File}},
 year = {2021}
}

@misc{ncbi,
 note = {\url{https://www.ncbi.nlm.nih.gov/}},
 title = {{National Center For Biotechnology Information}}
}

@article{needleman1970general,
 author = {Needleman, Saul B and Wunsch, Christian D},
 journal = {Journal of molecular biology},
 title = {{A General Method Applicable To The Search For Similarities In The Amino Acid Sequence Of Two Proteins}},
 year = {1970}
}

@article{ni2019ferroelectric,
 author = {Ni, Kai and Yin, Xunzhao and Laguna, Ann Franchesca and Joshi, Siddharth and Duenkel, Stefan and Trentzsch, Martin and M{\"u}ller, Johannes and Beyer, Sven and Niemier, Michael and Hu, Xiaobo Sharon and others},
 journal = {Nature Electronics},
 title = {{Ferroelectric Ternary Content-addressable Memory For One-shot Learning}},
 year = {2019}
}

@article{nikolayevskyy2016whole,
 author = {Nikolayevskyy, Vlad and Kranzer, Katharina and Niemann, Stefan and Drobniewski, Francis},
 journal = {Tuberculosis},
 title = {{Whole Genome Sequencing Of Mycobacterium Tuberculosis For Detection Of Recent Transmission And Tracing Outbreaks: A Systematic Review}},
 year = {2016}
}

@article{pagiamtzis2006content,
 author = {Pagiamtzis, Kostas and Sheikholeslami, Ali},
 journal = {IEEE journal of solid-state circuits},
 title = {{Content-addressable Memory (cam) Circuits And Architectures: A Tutorial And Survey}},
 year = {2006}
}

@article{payne2019bulkvis,
 author = {Payne, Alexander and Holmes, Nadine and Rakyan, Vardhman and Loose, Matthew},
 journal = {Bioinformatics},
 title = {{Bulkvis: A Graphical Viewer For Oxford Nanopore Bulk Fast5 Files}},
 year = {2019}
}

@article{perevsini2021nanopore,
 author = {Pere{\v{s}}{\'\i}ni, Peter and Bo{\v{z}}a, Vladim{\'\i}r and Brejov{\'a}, Bro{\v{n}}a and Vina{\v{r}}, Tom{\'a}{\v{s}}},
 journal = {Bioinformatics},
 title = {{Nanopore Base Calling On The Edge}},
 year = {2021}
}

@inproceedings{pinatubo,
 author = {Li, Shuangchen and Xu, Cong and Zou, Qiaosha and Zhao, Jishen and Lu, Yu and Xie, Yuan},
 booktitle = {Proceedings of the 53rd Annual Design Automation Conference},
 title = {{Pinatubo: A Processing-in-memory Architecture For Bulk Bitwise Operations In Emerging Non-volatile Memories}},
 year = {2016}
}

@article{pollard2018long,
 author = {Pollard, Martin O and Gurdasani, Deepti and Mentzer, Alexander J and Porter, Tarryn and Sandhu, Manjinder S},
 journal = {Human molecular genetics},
 title = {{Long Reads: Their Purpose And Place}},
 year = {2018}
}

@article{Prado-Martinez2013,
 author = {Prado-Martinez, Javier and Sudmant, Peter H. and Kidd, Jeffrey M. and Li, Heng and Kelley, Joanna L. and Lorente-Galdos, Belen and Veeramah, Krishna R. and Woerner, August E. and O'Connor, Timothy D. and Santpere, Gabriel and Cagan, Alexander and Theunert, Christoph and Casals, Ferran and Laayouni, Hafid and Munch, Kasper and Hobolth, Asger and Halager, Anders E. and Malig, Maika and Hernandez-Rodriguez, Jessica and Hernando-Herraez, Irene and Pr{\"{u}}fer, Kay and Pybus, Marc and Johnstone, Laurel and Lachmann, Michael and Alkan, Can and Twigg, Dorina and Petit, Natalia and Baker, Carl and Hormozdiari, Fereydoun and Fernandez-Callejo, Marcos and Dabad, Marc and Wilson, Michael L. and Stevison, Laurie and Camprub{\'{\i}}, Cristina and Carvalho, Tiago and Ruiz-Herrera, Aurora and Vives, Laura and Mele, Marta and Abello, Teresa and Kondova, Ivanela and Bontrop, Ronald E. and Pusey, Anne and Lankester, Felix and Kiyang, John A. and Bergl, Richard A. and Lonsdorf, Elizabeth and Myers, Simon and Ventura, Mario and Gagneux, Pascal and Comas, David and Siegismund, Hans and Blanc, Julie and Agueda-Calpena, Lidia and Gut, Marta and Fulton, Lucinda and Tishkoff, Sarah A. and Mullikin, James C. and Wilson, Richard K. and Gut, Ivo G. and Gonder, Mary Katherine and Ryder, Oliver A. and Hahn, Beatrice H. and Navarro, Arcadi and Akey, Joshua M. and Bertranpetit, Jaume and Reich, David and Mailund, Thomas and Schierup, Mikkel H. and Hvilsom, Christina and Andr{\'{e}}s, Aida M. and Wall, Jeffrey D. and Bustamante, Carlos D. and Hammer, Michael F. and Eichler, Evan E. and Marques-Bonet, Tomas},
 journal = {Nature},
 title = {{Great Ape Genetic Diversity And Population History}},
 year = {2013}
}

@article{Prohaska2019,
 author = {Prohaska, Ana and Racimo, Fernando and Schork, Andrew J and Sikora, Martin and Stern, Aaron J and Ilardo, Melissa and Allentoft, Morten Erik and Folkersen, Lasse and Buil, Alfonso and Moreno-Mayar, J Víctor and Korneliussen, Thorfinn and Geschwind, Daniel and Ingason, Andrés and Werge, Thomas and Nielsen, Rasmus and Willerslev, Eske},
 journal = {Cell},
 title = {{Human Disease Variation In The Light Of Population Genomics}},
 year = {2019}
}

@article{qiu2015whole,
 author = {Qiu, Shaofu and Li, Peng and Liu, Hongbo and Wang, Yong and Liu, Nan and Li, Chengyi and Li, Shenlong and Li, Ming and Jiang, Zhengjie and Sun, Huandong and others},
 journal = {Scientific Reports},
 title = {{Whole-genome Sequencing For Tracing The Transmission Link Between Two Ard Outbreaks Caused By A Novel Hadv Serotype 7 Variant, China}},
 year = {2015}
}

@inproceedings{ramachandra_ont-x_2021,
 author = {Ramachandra, C N and Nag, Anirban and Balasubramonion, Rajeev and Kalsi, Gurpreet and Pillai, Kamlesh and Subramoney, Sreenivas},
 booktitle = {2021 {IEEE} 29th {Annual} {International} {Symposium} on {Field}-{Programmable} {Custom} {Computing} {Machines} ({FCCM})},
 title = {{Ont-x: An Fpga Approach To Real-time Portable Genomic Analysis}},
 year = {2021}
}

@article{rang2018squiggle,
 author = {Rang, Franka J and Kloosterman, Wigard P and de Ridder, Jeroen},
 journal = {Genome biology},
 title = {{From Squiggle To Basepair: Computational Approaches For Improving Nanopore Sequencing Read Accuracy}},
 year = {2018}
}

@article{reuter2015high,
 author = {Reuter, Jason A and Spacek, Damek V and Snyder, Michael P},
 journal = {Molecular Cell},
 title = {{High-throughput Sequencing Technologies}},
 year = {2015}
}

@article{rivara-espasandin_nanopore_2022,
 author = {Rivara-Espasandín, Martín and Balestrazzi, Lucía and Dufort y Álvarez, Guillermo and Ochoa, Idoia and Seroussi, Gadiel and Smircich, Pablo and Sotelo-Silveira, José and Martín, Álvaro},
 journal = {Bioinformatics Advances},
 title = {{Nanopore Quality Score Resolution Can Be Reduced With Little Effect On Downstream Analysis}},
 year = {2022}
}

@article{roberts_reducing_2004,
 author = {Roberts, Michael and Hayes, Wayne and Hunt, Brian R. and Mount, Stephen M. and Yorke, James A.},
 journal = {Bioinformatics},
 title = {{Reducing Storage Requirements For Biological Sequence Comparison}},
 year = {2004}
}

@article{romiguier2014comparative,
 author = {Romiguier, J and Gayral, Philippe and Ballenghien, Marion and Bernard, Arnaud and Cahais, Vincent and Chenuil, A and Chiari, Ylenia and Dernat, R and Duret, L and Faivre, Nicolas and others},
 journal = {Nature},
 title = {{Comparative Population Genomics In Animals Uncovers The Determinants Of Genetic Diversity}},
 year = {2014}
}

@inproceedings{s_d_goenka_segalign_2020,
 author = {Goenka, Sneha D. and Turakhia, Yatish and Paten, Benedict and Horowitz, Mark},
 booktitle = {{SC20}: {International} {Conference} for {High} {Performance} {Computing}, {Networking}, {Storage} and {Analysis}},
 title = {{Segalign: A Scalable Gpu-based Whole Genome Aligner}},
 year = {2020}
}

@article{sahlin2021error,
 author = {Sahlin, Kristoffer and Medvedev, Paul},
 journal = {Nature communications},
 title = {{Error Correction Enables Use Of Oxford Nanopore Technology For Reference-free Transcriptome Analysis}},
 year = {2021}
}

@inproceedings{schleimer2003winnowing,
 author = {Schleimer, Saul and Wilkerson, Daniel S and Aiken, Alex},
 booktitle = {Proceedings of the 2003 ACM SIGMOD international conference on Management of data},
 title = {{Winnowing: Local Algorithms For Document Fingerprinting}},
 year = {2003}
}

@misc{Scrappie,
 author = { Oxford Nanopore Technology},
 journal = {GitHub repository},
 note = {\url{https://github.com/nanoporetech/scrappie }},
 title = {{Scrappie}}
}

@article{segerman2020most,
 author = {Segerman, Bo},
 journal = {Frontiers in Cellular and Infection Microbiology},
 title = {{The Most Frequently Used Sequencing Technologies And Assembly Methods In Different Time Segments Of The Bacterial Surveillance And Refseq Genome Databases}},
 year = {2020}
}

@inproceedings{senol2017nanopore,
 author = {Senol, Damla and Kim, Jeremie and Ghose, Saugata and Alkan, Can and Mutlu, Onur},
 booktitle = {Pacific Symposium on Biocomputing Poster Session},
 title = {{Nanopore Sequencing Technology And Tools: Computational Analysis Of The Current State, Bottlenecks And Future Directions}},
 year = {2017}
}

@article{sereika2022oxford,
 author = {Sereika, Mantas and Kirkegaard, Rasmus Hansen and Karst, S{\o}ren Michael and Michaelsen, Thomas Yssing and S{\o}rensen, Emil Aarre and Wollenberg, Rasmus Dam and Albertsen, Mads},
 journal = {Nature methods},
 title = {{Oxford Nanopore R10. 4 Long-read Sequencing Enables The Generation Of Near-finished Bacterial Genomes From Pure Cultures And Metagenomes Without Short-read Or Reference Polishing}},
 year = {2022}
}

@inproceedings{shafiee2016isaac,
 author = {A. Shafiee and Anirban Nag and N. Muralimanohar and Rajeev Balasubramonian and J. Strachan and Miao Hu and R. Williams and Vivek Srikumar},
 booktitle = {ISCA},
 title = {{Isaac: A Convolutional Neural Network Accelerator With In-situ Analog Arithmetic In Crossbars}},
 year = {2016}
}

@article{shafin2020nanopore,
 author = {Shafin, Kishwar and Pesout, Trevor and Lorig-Roach, Ryan and Haukness, Marina and Olsen, Hugh E and Bosworth, Colleen and Armstrong, Joel and Tigyi, Kristof and Maurer, Nicholas and Koren, Sergey and others},
 journal = {Nature biotechnology},
 title = {{Nanopore Sequencing And The Shasta Toolkit Enable Efficient De Novo Assembly Of Eleven Human Genomes}},
 year = {2020}
}

@article{singh2021fpga,
 author = {Singh, Gagandeep and Alser, Mohammed and Senol Cali, Damla and Diamantopoulos, Diamantopoulos and Gómez-Luna, Juan and Corporaal, Henk and Mutlu, Onur},
 journal = {IEEE Micro},
 title = {{Fpga-based Near-memory Acceleration Of Modern Data-intensive Applications}},
 year = {2021}
}

@article{smith1981identification,
 author = {Smith, Temple F and Waterman, Michael S and others},
 journal = {Journal of molecular biology},
 title = {{Identification Of Common Molecular Subsequences}},
 year = {1981}
}

@inproceedings{song2018graphr,
 author = {Song, Linghao and Zhuo, Youwei and Qian, Xuehai and Li, Hai and Chen, Yiran},
 booktitle = {2018 IEEE International Symposium on High Performance Computer Architecture (HPCA)},
 title = {{Graphr: Accelerating Graph Processing Using Reram}},
 year = {2018}
}

@article{sweeney2021rapid,
 author = {Sweeney, Nathaly M and Nahas, Shareef A and Chowdhury, Shimul and Batalov, Sergey and Clark, Michelle and Caylor, Sara and Cakici, Julie and Nigro, John J and Ding, Yan and Veeraraghavan, Narayanan and others},
 journal = {NPJ genomic medicine},
 title = {{Rapid Whole Genome Sequencing Impacts Care And Resource Utilization In Infants With Congenital Heart Disease}},
 year = {2021}
}

@article{tan2019experimental,
 author = {Tan, Ava J and Chatterjee, Korok and Zhou, Jiuren and Kwon, Daewoong and Liao, Yu-Hung and Cheema, Suraj and Hu, Chenming and Salahuddin, Sayeef},
 journal = {IEEE Electron Device Letters},
 title = {{Experimental Demonstration Of A Ferroelectric Hfo 2-based Content Addressable Memory Cell}},
 year = {2019}
}

@inproceedings{truong2021racer,
 author = {Truong, Minh SQ and Chen, Eric and Su, Deanyone and Shen, Liting and Glass, Alexander and Carley, L Richard and Bain, James A and Ghose, Saugata},
 booktitle = {MICRO-54: 54th Annual IEEE/ACM International Symposium on Microarchitecture},
 title = {{Racer: Bit-pipelined Processing Using Resistive Memory}},
 year = {2021}
}

@inproceedings{turakhia2018darwin,
 author = {Turakhia, Yatish and Bejerano, Gill and Dally, William J.},
 booktitle = {Proceedings of the {Twenty}-{Third} {International} {Conference} on {Architectural} {Support} for {Programming} {Languages} and {Operating} {Systems}},
 note = {Williamsburg, VA, USA},
 title = {{Darwin: A Genomics Co-processor Provides Up To 15,000x Acceleration On Long Read Assembly}},
 year = {2018}
}

@article{van2014ten,
 author = {van Dijk, Erwin L and Auger, H{\'e}l{\`e}ne and Jaszczyszyn, Yan and Claude Thermes},
 journal = {{Trends in Genetics}},
 title = {{Ten Years Of Next-generation Sequencing Technology}},
 year = {2014}
}

@article{van2018third,
 author = {van Dijk, Erwin L and Jaszczyszyn, Yan and Naquin, Delphine and Thermes, Claude},
 journal = {Trends in Genetics},
 title = {{The Third Revolution In Sequencing Technology}},
 year = {2018}
}

@article{wang2018novel,
 author = {Wang, Chengzhi and Zhang, Deming and Zeng, Lang and Deng, Erya and Chen, Jie and Zhao, Weisheng},
 journal = {IEEE Transactions on Circuits and Systems I: Regular Papers},
 title = {{A Novel Mtj-based Non-volatile Ternary Content-addressable Memory For High-speed, Low-power, And High-reliable Search Operation}},
 year = {2018}
}

@article{wang2019efficient,
 author = {Wang, Ou and Chin, Robert and Cheng, Xiaofang and Wu, Michelle Ka Yan and Mao, Qing and Tang, Jingbo and Sun, Yuhui and Anderson, Ellis and Lam, Han K and Chen, Dan and others},
 journal = {Genome research},
 title = {{Efficient And Unique Cobarcoding Of Second-generation Sequencing Reads From Long Dna Molecules Enabling Cost-effective And Accurate Sequencing, Haplotyping, And De Novo Assembly}},
 year = {2019}
}

@article{wang2020initial,
 author = {Wang, Fang and Huang, Shujia and Gao, Rongsui and Zhou, Yuwen and Lai, Changxiang and Li, Zhichao and Xian, Wenjie and Qian, Xiaobo and Li, Zhiyu and Huang, Yushan and others},
 journal = {Cell discovery},
 title = {{Initial Whole-genome Sequencing And Analysis Of The Host Genetic Contribution To Covid-19 Severity And Susceptibility}},
 year = {2020}
}

@article{wang2021nanopore,
 author = {Wang, Yunhao and Zhao, Yue and Bollas, Audrey and Wang, Yuru and Au, Kin Fai},
 journal = {Nature biotechnology},
 title = {{Nanopore Sequencing Technology, Bioinformatics And Applications}},
 year = {2021}
}

@article{weirather2017comprehensive,
 author = {Weirather, Jason L and de Cesare, Mariateresa and Wang, Yunhao and Piazza, Paolo and Sebastiano, Vittorio and Wang, Xiu-Jie and Buck, David and Au, Kin Fai},
 journal = {F1000Research},
 title = {{Comprehensive Comparison Of Pacific Biosciences And Oxford Nanopore Technologies And Their Applications To Transcriptome Analysis}},
 year = {2017}
}

@article{wick2019performance,
 author = {Wick, Ryan R and Judd, Louise M and Holt, Kathryn E},
 journal = {Genome biology},
 title = {{Performance Of Neural Network Basecalling Tools For Oxford Nanopore Sequencing}},
 year = {2019}
}

@article{wood2014kraken,
 author = {Wood, Derrick E and Salzberg, Steven L},
 journal = {Genome biology},
 title = {{Kraken: Ultrafast Metagenomic Sequence Classification Using Exact Alignments}},
 year = {2014}
}

@article{wood2019improved,
 author = {Wood, Derrick E and Lu, Jennifer and Langmead, Ben},
 journal = {Genome biology},
 title = {{Improved Metagenomic Analysis With Kraken 2}},
 year = {2019}
}

@article{wratten2021reproducible,
 author = {Wratten, Laura and Wilm, Andreas and G{\"o}ke, Jonathan},
 journal = {Nature Methods},
 title = {{Reproducible, Scalable, And Shareable Analysis Pipelines With Bioinformatics Workflow Managers}},
 year = {2021}
}

@inproceedings{wu2018fpga,
 author = {Wu, ZhongPan and Hammad, Karim and Mittmann, Robinson and Magierowski, Sebastian and Ghafar-Zadeh, Ebrahim and Zhong, Xiaoyong},
 booktitle = {2018 IEEE 61st International Midwest Symposium on Circuits and Systems (MWSCAS)},
 title = {{Fpga-based Dna Basecalling Hardware Acceleration}},
 year = {2018}
}

@article{wu_fpga-accelerated_2020,
 author = {Wu, Zhongpan and Hammad, Karim and Ghafar-Zadeh, Ebrahim and Magierowski, Sebastian},
 journal = {IEEE Transactions on Biomedical Circuits and Systems},
 title = {{Fpga-accelerated 3rd Generation Dna Sequencing}},
 year = {2020}
}

@inproceedings{wu_fpga_2022,
 author = {Wu, Zhongpan and Hammad, Karim and Beyene, Abel and Dawji, Yunus and Ghafar-Zadeh, Ebrahim and Magierowski, Sebastian},
 booktitle = {2022 20th {IEEE} {Interregional} {NEWCAS} {Conference} ({NEWCAS})},
 title = {{An Fpga Implementation Of A Portable Dna Sequencing Device Based On Risc-v}},
 year = {2022}
}

@article{xin2013accelerating,
 author = {Xin, Hongyi and Lee, Donghyuk and Hormozdiari, Farhad and Yedkar, Samihan and Mutlu, Onur and Alkan, Can},
 journal = {BMC Genomics},
 title = {{Accelerating Read Mapping With Fasthash}},
 year = {2013}
}

@article{xin2015shifted,
 author = {Xin, Hongyi and Greth, John and Emmons, John and Pekhimenko, Gennady and Kingsford, Carl and Alkan, Can and Mutlu, Onur},
 journal = {Bioinformatics},
 title = {{Shifted Hamming Distance: A Fast And Accurate Simd-friendly Filter To Accelerate Alignment Verification In Read Mapping}},
 year = {2015}
}

@inproceedings{xiu2021capacitive,
 author = {Xiu, Nuo and Chen, Yiming and Yin, Guodong and Ma, Xiaoyang and Yang, Huazhong and George, Sumitha and Li, Xueqing},
 booktitle = {Proceedings of the 2021 on Great Lakes Symposium on VLSI},
 title = {{Capacitive Content-addressable Memory: A Highly Reliable And Scalable Approach To Energy-efficient Parallel Pattern Matching Applications}},
 year = {2021}
}

@article{xu2021fast,
 author = {Xu, Zhimeng and Mai, Yuting and Liu, Denghui and He, Wenjun and Lin, Xinyuan and Xu, Chi and Zhang, Lei and Meng, Xin and Mafofo, Joseph and Zaher, Walid Abbas and others},
 journal = {Artificial Intelligence in the Life Sciences},
 title = {{Fast-bonito: A Faster Deep Learning Based Basecaller For Nanopore Sequencing}},
 year = {2021}
}

@article{yantir2017approximate,
 author = {Yantir, Hasan Erdem and Eltawil, Ahmed M and Kurdahi, Fadi J},
 journal = {ACM Transactions on Embedded Computing Systems (TECS)},
 title = {{Approximate Memristive In-memory Computing}},
 year = {2017}
}

@article{yeh_msrcall_2022,
 author = {Yeh, Yang-Ming and Lu, Yi-Chang},
 journal = {Bioinformatics},
 title = {{Msrcall: A Multi-scale Deep Neural Network To Basecall Oxford Nanopore Sequences}},
 year = {2022}
}

@article{yelagandula2021multiplexed,
 author = {Yelagandula, Ramesh and Bykov, Aleksandr and Vogt, Alexander and Heinen, Robert and {\"O}zkan, Ezgi and Strobl, Marcus Martin and Baar, Juliane Christina and Uzunova, Kristina and Hajdusits, Bence and Kordic, Darja and others},
 journal = {Nature Communications},
 title = {{Multiplexed Detection Of Sars-cov-2 And Other Respiratory Infections In High Throughput By Sarseq}},
 year = {2021}
}

@inproceedings{yin2017design,
 author = {Yin, Xunzhao and Niemier, Michael and Hu, X Sharon},
 booktitle = {Design, Automation \& Test in Europe Conference \& Exhibition (DATE), 2017},
 title = {{Design And Benchmarking Of Ferroelectric Fet Based Tcam}},
 year = {2017}
}

@article{yin2018ultra,
 author = {Yin, Xunzhao and Ni, Kai and Reis, Dayane and Datta, Suman and Niemier, Michael and Hu, Xiaobo Sharon},
 journal = {IEEE Transactions on Circuits and Systems II: Express Briefs},
 title = {{An Ultra-dense 2fefet Tcam Design Based On A Multi-domain Fefet Model}},
 year = {2018}
}

@article{yin2020fecam,
 author = {Yin, Xunzhao and Li, Chao and Huang, Qingrong and Zhang, Li and Niemier, Michael and Hu, Xiaobo Sharon and Zhuo, Cheng and Ni, Kai},
 journal = {IEEE Transactions on Electron Devices},
 title = {{Fecam: A Universal Compact Digital And Analog Content Addressable Memory Using Ferroelectric}},
 year = {2020}
}

@article{yuan2021forms,
 author = {Yuan, Geng and Behnam, Payman and Li, Zhengang and Shafiee, Ali and Lin, Sheng and Ma, Xiaolong and Liu, Hang and Qian, Xuehai and Bojnordi, Mahdi Nazm and Wang, Yanzhi and others},
 journal = {arXiv preprint arXiv:2106.09144},
 title = {{Forms: Fine-grained Polarized Reram-based In-situ Computation For Mixed-signal Dnn Accelerator}},
 year = {2021}
}

@article{zeng_causalcall_2020,
 author = {Zeng, Jingwen and Cai, Hongmin and Peng, Hong and Wang, Haiyan and Zhang, Yue and Akutsu, Tatsuya},
 journal = {Frontiers in Genetics},
 title = {{Causalcall: Nanopore Basecalling Using A Temporal Convolutional Network}},
 year = {2020}
}

@article{zhang2021real,
 author = {Zhang, Haowen and Li, Haoran and Jain, Chirag and Cheng, Haoyu and Au, Kin Fai and Li, Heng and Aluru, Srinivas},
 journal = {Bioinformatics},
 title = {{Real-time Mapping Of Nanopore Raw Signals}},
 year = {2021}
}

@article{Zhao2019RFAccA3,
 author = {Lei Zhao and Quan Deng and Youtao Zhang and J. Yang},
 journal = {Proceedings of the ACM International Conference on Supercomputing},
 title = {{Rfacc: A 3d Reram Associative Array Based Random Forest Accelerator}},
 year = {2019}
}

@article{zokaee2018aligner,
 author = {Zokaee, Farzaneh and Zarandi, Hamid R and Jiang, Lei},
 journal = {IEEE Computer Architecture Letters},
 title = {{Aligner: A Process-in-memory Architecture For Short Read Alignment In Rerams}},
 year = {2018}
}

@inproceedings{zokaee2019finder,
 author = {Zokaee, Farzaneh and Zhang, Mingzhe and Jiang, Lei},
 booktitle = {2019 28th International Conference on Parallel Architectures and Compilation Techniques (PACT)},
 title = {{Finder: Accelerating Fm-index-based Exact Pattern Matching In Genomic Sequences Through Reram Technology}},
 year = {2019}
}


@inproceedings{khalifa_filtpim_2021,
	title = {{FiltPIM}: {In}-{Memory} {Filter} for {DNA} {Sequencing}},
	doi = {10.1109/ICECS53924.2021.9665570},
	booktitle = {2021 28th {IEEE} {International} {Conference} on {Electronics}, {Circuits}, and {Systems} ({ICECS})},
	author = {Khalifa, Marcel and Ben-Hur, Rotem and Ronen, Ronny and Leitersdorf, Orian and Yavits, Leonid and Kvatinsky, Shahar},
	year = {2021},
	pages = {1--4},
}

@article{chowdhury_dna_2020,
	title = {A {DNA} {Read} {Alignment} {Accelerator} {Based} on {Computational} {RAM}},
	volume = {6},
	doi = {10.1109/JXCDC.2020.2987527},
	number = {1},
	journal = {IEEE Journal on Exploratory Solid-State Computational Devices and Circuits},
	author = {Chowdhury, Zamshed I. and Zabihi, Masoud and Khatamifard, S. Karen and Zhao, Zhengyang and Resch, Salonik and Razaviyayn, Meisam and Wang, Jian-Ping and Sapatnekar, Sachin S. and Karpuzcu, Ulya R.},
	year = {2020},
	pages = {80--88},
}

@inproceedings{huangfu_radar_2018,
	address = {New York, NY, USA},
	series = {{DAC} '18},
	title = {{RADAR}: {A} {3D}-{ReRAM} {Based} {DNA} {Alignment} {Accelerator} {Architecture}},
	isbn = {978-1-4503-5700-5},
	url = {https://doi.org/10.1145/3195970.3196098},
	doi = {10.1145/3195970.3196098},
	booktitle = {Proceedings of the 55th {Annual} {Design} {Automation} {Conference}},
	publisher = {Association for Computing Machinery},
	author = {Huangfu, Wenqin and Li, Shuangchen and Hu, Xing and Xie, Yuan},
	year = {2018},
}


